Adam in Private: Secure and Fast Training of Deep Neural Networks with Adaptive Moment Estimation

Privacy-preserving machine learning (PPML) aims at enabling machine learning (ML) algorithms to be used on sensitive data. We contribute to this line of research by proposing a framework that allows efficient and secure evaluation of full-fledged state-of-the-art ML algorithms via secure multi-party computation (MPC). This is in contrast to most prior works, which substitute ML algorithms with approximated "MPC-friendly" variants. A drawback of the latter approach is that fine-tuning of the combined ML and MPC algorithms is required, which might lead to less efficient algorithms or inferior quality ML. This is an issue for secure deep neural networks (DNN) training in particular, as this involves arithmetic algorithms thought to be "MPC-unfriendly", namely, integer division, exponentiation, inversion, and square root. In this work, we propose secure and efficient protocols for the above seemingly MPC-unfriendly computations. Our protocols are three-party protocols in the honest-majority setting, and we propose both passively secure and actively secure with abort variants. A notable feature of our protocols is that they simultaneously provide high accuracy and efficiency. This framework enables us to efficiently and securely compute modern ML algorithms such as Adam and the softmax function "as is", without resorting to approximations. As a result, we obtain secure DNN training that outperforms state-of-the-art three-party systems; our full training is up to 6.7 times faster than just the online phase of the recently proposed FALCON@PETS'21 on a standard benchmark network. We further perform measurements on real-world DNNs, AlexNet and VGG16. The performance of our framework is up to a factor of about 12-14 faster for AlexNet and 46-48 faster for VGG16 to achieve an accuracy of 70% and 75%, respectively, when compared to FALCON.

==> kikuchistyle.tex <==
%\nvewcommand{\keywords}[1]{\par\addvspace\baselineskip
%\noindent\keywordname\enspace\ignorespaces#1}
\usepackage{amssymb, mathrsfs, hhline, url}
%\usepackage[cmex10]{amsmath}
%\usepackage{amsmath}
%%%%%%%%%%%%%%%		calligraphy		%%%%%%%%%%%%%%%%%
\def\A{{\mathcal{A}}}
\def\B{{\mathcal{B}}}
\def\C{{\mathcal{C}}}
\def\D{{\mathcal{D}}}
\def\E{{\mathcal{E}}}
\def\F{{\mathcal{F}}}
\def\G{{\mathcal{G}}}
\def\H{{\mathcal{H}}}
\def\I{{\mathcal{I}}}
\def\J{{\mathcal{J}}}
\def\Kset{{\mathcal{K}}}
\def\L{{\mathcal{L}}}
\def\M{{\mathcal{M}}}
\def\N{{\mathcal{N}}}
\def\O{{\mathcal{O}}}
\def\P{{\mathcal{P}}}
\def\Q{{\mathcal{Q}}}
\def\R{{\mathcal{R}}}
\def\S{{\mathcal{S}}}
\def\T{{\mathcal{T}}}
\def\U{{\mathcal{U}}}
\def\V{{\mathcal{V}}}
\def\W{{\mathcal{W}}}
\def\X{{\mathcal{X}}}
\def\Y{{\mathcal{Y}}}
\def\Z{{\mathcal{Z}}}

\newcommand{\FF}{\mathbb{F}}
\newcommand{\finput}{{\F_{\rm input}}}
\newcommand{\abort}{{\sf abort}}
\newcommand{\frand}{{\F_{\rm rand}}}
\newcommand{\xfrand}{{\widehat{\F}_{\rm rand}}}
\newcommand{\fmult}{\F_{\rm mult}}
\newcommand{\xfmult}{\widehat{\F}_{\rm mult}}
\newcommand{\fproduct}{\F_{\rm product}}
\newcommand{\xfproduct}{\widehat{\F}_{\rm product}}
\newcommand{\Open}{{\sf Open}}
\newcommand{\fcheckzero}{{\F_{\rm checkZero}}}
\newcommand{\xfcheckzero}{{\widehat{\F}_{\rm checkZero}}}
\newcommand{\Reconstruct}{{\sf Reconstruct}}
\newcommand{\fcoin}{{\F_{\rm coin}}}
\newcommand{\xfcoin}{{\widehat{\F}_{\rm coin}}}
%--------------------------------
% Utilities
%--------------------------------
\newcommand{\keys}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\orac}[1]{\text{\sc #1}}
\newcommand{\scheme}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\algo}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\protocol}[1]{\ensuremath{\textsc{#1}}}
\newcommand{\events}[1]{\textsl{#1}}
\newcommand{\attack}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\ahyph}{\attack{\mathchar`-}}
\newcommand{\security}[1]{\ensuremath{\textsc{#1}}}
\newcommand{\game}[1]{\ensuremath{\textsc{#1}}}
\newcommand{\shyph}{\security{-}}


%%%%%%%%%%%%   set  %%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\newcommand{\etal}{{et~al.~}}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\newcommand{\func}[1]{\ensuremath{\mathop{\mathrm{#1}}\nolimits}}
\newcommand{\sett}[1]{\ensuremath{\mathbb{#1}}}

\newcommand{\Aset}{\ensuremath{\sett{A}}}
\newcommand{\Bset}{\ensuremath{\sett{B}}}
\newcommand{\Cset}{\ensuremath{\sett{C}}}
\newcommand{\Dset}{\ensuremath{\sett{D}}}
\newcommand{\Eset}{\ensuremath{\sett{E}}}
\newcommand{\Fset}{\ensuremath{\sett{F}}}
\newcommand{\Gset}{\ensuremath{\sett{G}}}
\newcommand{\Hset}{\ensuremath{\sett{H}}}
\newcommand{\Iset}{\ensuremath{\sett{I}}}
\newcommand{\Jset}{\ensuremath{\sett{J}}}
\newcommand{\Ksetset}{\ensuremath{\sett{K}}}
\newcommand{\xKsetset}{\ensuremath{\widehat{\sett{K}}}}
\newcommand{\Lset}{\ensuremath{\sett{L}}}
\newcommand{\Mset}{\ensuremath{\sett{M}}}
\newcommand{\Nset}{\ensuremath{\sett{N}}}
\newcommand{\Oset}{\ensuremath{\sett{O}}}
\newcommand{\Pset}{\ensuremath{\sett{P}}}
\newcommand{\Qset}{\ensuremath{\sett{Q}}}
\newcommand{\Rset}{\ensuremath{\sett{R}}}
\newcommand{\Sset}{\ensuremath{\sett{S}}}
\newcommand{\Tset}{\ensuremath{\sett{T}}}
\newcommand{\Uset}{\ensuremath{\sett{U}}}
\newcommand{\Vset}{\ensuremath{\sett{V}}}
\newcommand{\Wset}{\ensuremath{\sett{W}}}
\newcommand{\Xset}{\ensuremath{\sett{X}}}
\newcommand{\Yset}{\ensuremath{\sett{Y}}}
\newcommand{\Zset}{\ensuremath{\sett{Z}}}

\newcommand{\Amat}{\ensuremath{\mat{A}}}
\newcommand{\Bmat}{\ensuremath{\mat{B}}}
\newcommand{\Cmat}{\ensuremath{\mat{C}}}
\newcommand{\Dmat}{\ensuremath{\mat{D}}}
\newcommand{\Emat}{\ensuremath{\mat{E}}}
\newcommand{\Fmat}{\ensuremath{\mat{F}}}
\newcommand{\Gmat}{\ensuremath{\mat{G}}}
\newcommand{\Hmat}{\ensuremath{\mat{H}}}
\newcommand{\Imat}{\ensuremath{\mat{I}}}
\newcommand{\Jmat}{\ensuremath{\mat{J}}}
\newcommand{\Ksetmat}{\ensuremath{\mat{K}}}
\newcommand{\Lmat}{\ensuremath{\mat{L}}}
\newcommand{\Mmat}{\ensuremath{\mat{M}}}
\newcommand{\Nmat}{\ensuremath{\mat{N}}}
\newcommand{\Omat}{\ensuremath{\mat{O}}}
\newcommand{\Pmat}{\ensuremath{\mat{P}}}
\newcommand{\Qmat}{\ensuremath{\mat{Q}}}
\newcommand{\Rmat}{\ensuremath{\mat{R}}}
\newcommand{\Smat}{\ensuremath{\mat{S}}}
\newcommand{\Tmat}{\ensuremath{\mat{T}}}
\newcommand{\Umat}{\ensuremath{\mat{U}}}
\newcommand{\Vmat}{\ensuremath{\mat{V}}}
\newcommand{\Wmat}{\ensuremath{\mat{W}}}
\newcommand{\Xmat}{\ensuremath{\mat{X}}}
\newcommand{\Ymat}{\ensuremath{\mat{Y}}}
\newcommand{\Zmat}{\ensuremath{\mat{Z}}}

\newcommand{\GF}{\func{GF}}
%\newcommand{\Zp}{{\Zset}/{p}{\Zset}}
%\newcommand{\Zq}{{\Zset}/{q}{\Zset}}
%\newcommand{\Zn}{{\Zset}/{n}{\Zset}}
%\newcommand{\ZN}{{\Zset}/{N}{\Zset}}
\newcommand{\Zp}{{{\Zset}_{p}}}
\newcommand{\Zq}{{{\Zset}_{q}}}
\newcommand{\Zn}{{{\Zset}_{n}}}
\newcommand{\ZN}{{{\Zset}_{N}}}
\newcommand{\Zl}{{{\Zset}_{\ell}}}
\newcommand{\Ztwo}{{{\Zset}_{2}}}

\newcommand{\Fp}{{{\Fset}_p}}


%---------------------------------------
% others
%---------------------------------------
\newcommand{\cycl}[1]{\left\langle{#1}\right\rangle} %%%% usage $\cycl{g}$ 
\newcommand{\lsb}{\func{lsb}}
\newcommand{\msb}{\func{msg}}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\card}[1]{\left\lvert{#1}\right\rvert}
% \newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\share}[1]{[{#1}]}
\newcommand{\sharee}[1]{[\![{#1}]\!]}
\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\eqq}{\stackrel{\rm ?}{=}}
\newcommand{\indp}{\stackrel{\rm p}{\approx}}
\newcommand{\inds}{\stackrel{\rm s}{\approx}}
\newcommand{\indc}{\stackrel{\rm c}{\approx}}
\newcommand{\inr}{\in_{\mbox{\tiny R}}}
\newcommand{\getsr}{\gets_{\mbox{\tiny R}}}
\newcommand{\bit}{\{0,1\}}
\newcommand{\poly}{\func{poly}}
\renewcommand{\vec}[1]{\overrightarrow{#1}}
\newcommand{\sss}[1]{\scriptscriptstyle{#1}}
\newcommand{\texts}[1]{\textrm{\tiny #1}}
\newcommand{\essinf}{\text{ess inf}}
\newcommand{\prob}[1]{\Pr \left[ #1 \right]}
\def\blackslug
{\hbox{\hskip 1pt\vrule width 8pt height 8pt depth 1.5pt\hskip 1pt}}
\def\qed{\quad\blackslug\lower 8.5pt\null\par}
\def\qqed{$\Box$}
\def\bs{\backslash}
\newcommand{\wwedge}{~\wedge~}
\newcommand{\Group}{\ensuremath{\mathscr{G}}}
\newcommand{\Ring}{\ensuremath{\mathscr{R}}}
\newcommand{\Field}{\ensuremath{\mathscr{F}}}
\newcommand{\Seed}{\ensuremath{\mathscr{S}}}

%%%%%%%%%%%%   displaystyle   %%%%%%%%%%%%%%
\newcommand{\ds}[1]{{\displaystyle {#1}}}
\newcommand{\dsum}{\displaystyle \sum}
\newcommand{\dprod}{\displaystyle \prod}
\newcommand{\dmin}{\displaystyle \min}
\newcommand{\dmax}{\displaystyle \max}
\newcommand{\dint}{\displaystyle \int}


%----------------------------------
%Index/parameter
%----------------------------------
%Keys
% \newcommand{\id}{\keys{id}}
\newcommand{\ID}{\keys{ID}}
\newcommand{\did}{\keys{d_{\id}}}
\newcommand{\ck}{\keys{ck}}
\newcommand{\ek}{\keys{ek}}
\newcommand{\EK}{\keys{EK}}
\newcommand{\dk}{\keys{dk}}
\newcommand{\DK}{\keys{DK}}
% \newcommand{\vk}{\keys{vk}}
\newcommand{\sk}{\keys{sk}}
\newcommand{\ovk}{\keys{ovk}}
\newcommand{\osk}{\keys{osk}}
% \newcommand{\pk}{\keys{pk}}
\newcommand{\tk}{\keys{tk}}
\newcommand{\hk}{\keys{hk}}
\newcommand{\usk}{\keys{usk}}
\newcommand{\upk}{\keys{upk}}
\newcommand{\gsk}{\keys{g}\kern-.05em\keys{sk}}
\newcommand{\gpk}{\keys{gpk}}
\newcommand{\rsk}{\keys{rsk}}
\newcommand{\rpk}{\keys{rpk}}
\newcommand{\tpk}{\keys{tpk}}
\newcommand{\tsk}{\keys{tsk}}
\newcommand{\msk}{\keys{msk}}
\newcommand{\rk}{\keys{rk}}
\newcommand{\pp}{\keys{pp}}
\newcommand{\pars}{\keys{pars}}
\newcommand{\cipher}{\keys{ct}}
\newcommand{\msg}{\keys{m}}
\newcommand{\PK}{\keys{PK}}
\newcommand{\SK}{\keys{SK}}
\newcommand{\sid}{\keys{sid}}
\newcommand{\qid}{\keys{qid}}
\newcommand{\pid}{\keys{pid}}
\newcommand{\key}{\keys{key}}
\newcommand{\params}{\keys{params}}
\newcommand{\crs}{\keys{crs}}



%----------------------------------
%Index/parameter
%----------------------------------
\newcommand{\Index}{\mathcal{I}}
\newcommand{\spar}{\lambda}
%----------------------------------
%hash
%----------------------------------
\newcommand{\HashH}{\mathcal{H}}
\newcommand{\HashF}{\mathcal{F}}
%----------------------------------
%chameleon hash function/trapdoor commitment
%----------------------------------
\newcommand{\CH}{\mathcal{CH}}
\newcommand{\CHGen}{\algo{CHGen}}
\newcommand{\CHEval}{\algo{CHEval}}
\newcommand{\CHColl}{\algo{CHColl}}
%---------------------------------
%advantages, distributions, experiments
%---------------------------------
\newcommand{\Adv}{\ensuremath{\mathsf{Adv}}}
\newcommand{\Succ}{\ensuremath{\mathsf{Succ}}}
\newcommand{\EXEC}{\game{EXEC}}
\newcommand{\Dist}{\game{Dist}}
\newcommand{\Expt}{\game{Expt}}
\newcommand{\View}{\game{View}}
\newcommand{\Output}{\game{Output}}
%---------------------------------
%negligibility
%---------------------------------
\newcommand{\negl}{\ensuremath{\mathsf{negl}}}
\newcommand{\nonnegl}{\mbox\ensuremath{\mathsf{non-negl}}}
%----------------------------------
%  values
%----------------------------------
\newcommand{\val}{\ensuremath{\mathsf{val}}}
%----------------------------------
%  events
%----------------------------------
\newcommand{\allow}{\ensuremath{\events{allow}}}
\newcommand{\deny}{\ensuremath{\events{deny}}}
\newcommand{\success}{\ensuremath{\events{success}}}
\newcommand{\fail}{\ensuremath{\events{fail}}}
\newcommand{\accept}{\ensuremath{\events{accept}}}
\newcommand{\reject}{\ensuremath{\events{reject}}}
\newcommand{\correct}{\ensuremath{\events{correct}}}
\newcommand{\wrong}{\ensuremath{\events{wrong}}}
\newcommand{\true}{\ensuremath{\events{true}}}
\newcommand{\false}{\ensuremath{\events{false}}}
\newcommand{\good}{\ensuremath{\events{good}}}
%----------------------------------
%  schemes
%----------------------------------
\newcommand{\Schemepi}{\rm{\Pi}}

\newcommand{\Gen}{\algo{Gen}}
\newcommand{\KsetGen}{\algo{KGen}}
\newcommand{\CRSGen}{\algo{CRSGen}}
\newcommand{\Setup}{\algo{Setup}}
\newcommand{\Enc}{\algo{Enc}}
\newcommand{\Dec}{\algo{Dec}}
%
\newcommand{\PKE}{\scheme{PKE}}
\newcommand{\PGen}{\algo{PKE.Gen}}
\newcommand{\PDec}{\algo{PKE.Dec}}
\newcommand{\PEnc}{\algo{PKE.Enc}}
%
\newcommand{\KsetEM}{\scheme{KEM}}
\newcommand{\KsetEMGen}{\algo{KEM.Gen}}
\newcommand{\KsetEMEnc}{\algo{KEM.Enc}}
\newcommand{\KsetEMDec}{\algo{KEM.Dec}}
%
\newcommand{\DEM}{\scheme{DEM}}
\newcommand{\DEMEnc}{\algo{DEM.Enc}}
\newcommand{\DEMDec}{\algo{DEM.Dec}}
%
\newcommand{\IBE}{\scheme{IBE}}
\newcommand{\IBESet}{\algo{IBE.Setup}}
\newcommand{\IBEGen}{\algo{IBE.Gen}}
\newcommand{\IBEEnc}{\algo{IBE.Enc}}
\newcommand{\IBEDec}{\algo{IBE.Dec}}
%
\newcommand{\Sig}{\algo{Sign}}
\newcommand{\Ver}{\algo{Ver}}
%
\newcommand{\SIG}{\scheme{SIG}}
\newcommand{\SIGGen}{\algo{SIG.Gen}}
\newcommand{\SIGSig}{\algo{SIG.Sign}}
\newcommand{\SIGVer}{\algo{SIG.Ver}}
%
\newcommand{\ZK}{\algo{ZK}}
%
\renewcommand{\SS}{\scheme{SS}}
\newcommand{\Share}{\algo{Share}}
\newcommand{\Reconst}{\algo{Rec}}
\newcommand{\Sharee}{\widehat{\algo{Share}}}
\newcommand{\Reconstt}{\widehat{\algo{Rec}}}
\newcommand{\Convert}{\algo{Convert}}
\newcommand{\SShare}{\algo{SS.Share}}
\newcommand{\SReconst}{\algo{SS.Rec}}
%
%
%

\newtheorem{myprotocol}[theorem]{PROTOCOL}{\bf}{}            %
\newtheorem{myfigure}[theorem]{FIGURE}{\bf}{} 
\newtheorem{myfunctionality}[theorem]{FUNCTIONALITY}{\bf}{}           %

\newcommand{\BPR}{\begin{myprotocol}}   \newcommand{\EPR}{\end{myprotocol}}
\newcommand{\ourfigg}[5]{
{\begin{figure}[#4]
\begin{center}
\framebox[\width][c]{
    \small
    \hbox{\quad
    \begin{varwidth}[c]{0.9\textwidth}
    %\begin{center}
    \begin{myfigure}
    [#1]
    \label{#2}
    \end{myfigure}
    %\end{center}
    
    #5
    \end{varwidth}
    \quad}
    }
    \begin{center} #3 \end{center}
    \vspace{-6ex}
\end{center}
\end{figure}
} }


% USAGE: \ourfig{TITLE}{LABEL}{CAPTION}{BODY}
\newcommand{\ourfig}[4]{\ourfigg{#1}{#2}{#3}{htb}{#4}}
\newcommand{\ourfigH}[4]{\ourfigg{#1}{#2}{#3}{H}{#4}}


\newcommand{\prott}[5]{
{\begin{figure}[#4]
\begin{center}
\framebox[\columnwidth][c]{
    \small
    \hbox{\quad
    \begin{varwidth}[c]{0.95\columnwidth}
    %\begin{center}
    \begin{myprotocol}
    [#1]
    \label{#2}
    \end{myprotocol}
    %\end{center}
    
    #5
    \end{varwidth}
    \quad}
    }
    \begin{center} #3 \end{center}
    \vspace{-6ex}
\end{center}
\end{figure}
} }

\newcommand{\prottcont}[3]{
{\begin{figure}[#3]
\begin{center}
\framebox[\width][c]{
    \small
    \hbox{\quad
    \begin{varwidth}[c]{0.9\textwidth}
    %\begin{center}
    \noindent{\bf #1} \vspace{2ex}
    %\end{center}
    
    #2
    \end{varwidth}
    \quad}
    }
    %\vspace{-4ex}
\end{center}
\end{figure}
} }

\newcommand{\protm}[5]{
{\begin{figure*}[#4]
\begin{center}
\framebox[\width][c]{
    \hbox{\quad
    \begin{varwidth}[c]{0.95\textwidth}
    %\begin{center}
    \begin{myprotocol}
    [#1]
    \label{#2}
    \end{myprotocol}
    %\end{center}

    #5
    \end{varwidth}
    \quad}
    }
    \begin{center} #3 \end{center}
    \vspace{-4ex}
\end{center}
\end{figure*}
} }

\newcommand{\functionality}[5]{
{\begin{figure}[#4]
\begin{center}
\framebox[\width][c]{
    \small
    \hbox{\quad
    \begin{varwidth}[c]{0.9\columnwidth}
    %\begin{center}
    \begin{myfunctionality}
    [#1]
    \label{#2}
    \end{myfunctionality}
    %\end{center}
    \vspace{-3ex}
    #5
    \end{varwidth}
    \quad}
    }
    \begin{center} #3 \end{center}
    \vspace{-6ex}
\end{center}
\end{figure}
} }

\newcommand{\vals}[1]{{\sf val}(\share{#1})}
%\newcommand{\val}[1]{{\sf val}(#1)}

% USAGE: \function{TITLE}{LABEL}{CAPTION}{BODY}
\newcommand{\function}[4]{\functionality{#1}{#2}{#3}{htb}{#4}}
\newcommand{\functionH}[4]{\functionality{#1}{#2}{#3}{H}{#4}}

% USAGE: \prot{TITLE}{LABEL}{CAPTION}{BODY}
\newcommand{\prot}[4]{\prott{#1}{#2}{#3}{htb}{#4}}
\newcommand{\protH}[4]{\prott{#1}{#2}{#3}{H}{#4}}
\newcommand{\protp}[5]{\prott{#1}{#2}{#3}{#4}{#5}}
\newcommand{\protM}[4]{\protm{#1}{#2}{#3}{ht}{#4}}
%
% \newcommand{\Shamir}{\scheme{Shamir}}
% \newcommand{\ShaShare}{\algo{Shamir.Share}}
% \newcommand{\ShaReconst}{\algo{Shamir.Rec}}
% %
% \newcommand{\Hom}{\scheme{Hom}}
% \newcommand{\HShare}{\algo{Hom.Share}}
% \newcommand{\HReconst}{\algo{Hom.Rec}}
% %
% \newcommand{\Linear}{\scheme{Lin}}
% \newcommand{\LShare}{\algo{Lin.Share}}
% \newcommand{\LReconst}{\algo{Lin.Rec}}
% %
% \newcommand{\Ramp}{\scheme{Ramp}}
% \newcommand{\RShare}{\algo{Ramp.Share}}
% \newcommand{\RReconst}{\algo{Ramp.Rec}}
% \newcommand{\RConvert}{\algo{Ramp.Convert}}
% %
% \newcommand{\IDA}{\scheme{IDA}}
% \newcommand{\ISplit}{\algo{IDA.Split}}
% \newcommand{\IReconst}{\algo{IDA.Rec}}
% %
% \newcommand{\PRG}{\ensuremath{\phi}}
% %

% %%%%%%%% security notion %%%%%%%%%
% \newcommand{\Goal}{\security{Goal}}
% \newcommand{\OT}{\security{OT}}
% \newcommand{\IND}{\security{IND}}
% \newcommand{\ANO}{\security{ANO}}
% \newcommand{\AI}{\security{AI}}
% \newcommand{\INDPA}{\security{INDPA}}
% \newcommand{\OW}{\security{OW}}
% \newcommand{\NM}{\security{NM}}
% \newcommand{\SNM}{\security{SNM}}
% \newcommand{\CNM}{\security{CNM}}
% %
% \newcommand{\ATK}{\security{ATK}}
% \newcommand{\CPA}{\security{CPA}}
% \newcommand{\CCA}{\security{CCA}}
% \newcommand{\CCAa}{\security{CCA1}}
% \newcommand{\CCAb}{\security{CCA2}}
% \newcommand{\SCCA}{\security{SCCA}}
% %-----------------------------------------
% % OW
% \newcommand{\owatk}{\ow\ahyph\atk}
% \newcommand{\owcpa}{\ow\ahyph\cpa}
% \newcommand{\owccaa}{\ow\ahyph\ccaa}
% \newcommand{\owccab}{\ow\ahyph\ccab}
% \newcommand{\OWATK}{\OW\shyph\ATK}
% \newcommand{\OWCPA}{\OW\shyph\CPA}
% \newcommand{\OWCCAa}{\OW\shyph\CCAa}
% \newcommand{\OWCCAb}{\OW\shyph\CCAb}
% % IND 
% \newcommand{\indatk}{\ind\ahyph\atk}
% \newcommand{\indcpa}{\ind\ahyph\cpa}
% \newcommand{\indccaa}{\ind\ahyph\ccaa}
% \newcommand{\indccab}{\ind\ahyph\ccab}
% \newcommand{\INDATK}{\IND\shyph\ATK}
% \newcommand{\INDCPA}{\IND\shyph\CPA}
% \newcommand{\INDCCAa}{\IND\shyph\CCAa}
% \newcommand{\INDCCAb}{\IND\shyph\CCAb}
% % ANO
% \newcommand{\anoatk}{\ano\ahyph\atk}
% \newcommand{\anocpa}{\ano\ahyph\cpa}
% \newcommand{\anoccaa}{\ano\ahyph\ccaa}
% \newcommand{\anoccab}{\ano\ahyph\ccab}
% \newcommand{\ANOATK}{\ANO\shyph\ATK}
% \newcommand{\ANOCPA}{\ANO\shyph\CPA}
% \newcommand{\ANOCCAa}{\ANO\shyph\CCAa}
% \newcommand{\ANOCCAb}{\ANO\shyph\CCAb}
% % AI
% \newcommand{\aiatk}{\ai\ahyph\atk}
% \newcommand{\aicpa}{\ai\ahyph\cpa}
% \newcommand{\aiccaa}{\ai\ahyph\ccaa}
% \newcommand{\aiccab}{\ai\ahyph\ccab}
% \newcommand{\AIATK}{\AI\shyph\ATK}
% \newcommand{\AICPA}{\AI\shyph\CPA}
% \newcommand{\AICCA}{\AI\shyph\CCA}
% \newcommand{\AICCAa}{\AI\shyph\CCAa}
% \newcommand{\AICCAb}{\AI\shyph\CCAb}
% % NM
% \newcommand{\nmatk}{\nm\ahyph\atk}
% \newcommand{\nmcpa}{\nm\ahyph\cpa}
% \newcommand{\nmccaa}{\nm\ahyph\ccaa}
% \newcommand{\nmccab}{\nm\ahyph\ccab}
% \newcommand{\NMATK}{\NM\shyph\ATK}
% \newcommand{\NMCPA}{\NM\shyph\CPA}
% \newcommand{\NMCCAa}{\NM\shyph\CCAa}
% \newcommand{\NMCCAb}{\NM\shyph\CCAb}
% % SNM
% \newcommand{\snmatk}{\snm\ahyph\atk}
% \newcommand{\snmcpa}{\snm\ahyph\cpa}
% \newcommand{\snmccaa}{\snm\ahyph\ccaa}
% \newcommand{\snmccab}{\snm\ahyph\ccab}
% \newcommand{\SNMATK}{\SNM\shyph\ATK}
% \newcommand{\SNMCPA}{\SNM\shyph\CPA}
% \newcommand{\SNMCCAa}{\SNM\shyph\CCAa}
% \newcommand{\SNMCCAb}{\SNM\shyph\CCAb}
% % CNM
% \newcommand{\cnmatk}{\cnm\ahyph\atk}
% \newcommand{\cnmcpa}{\cnm\ahyph\cpa}
% \newcommand{\cnmccaa}{\cnm\ahyph\ccaa}
% \newcommand{\cnmccab}{\cnm\ahyph\ccab}
% \newcommand{\CNMATK}{\CNM\shyph\ATK}
% \newcommand{\CNMCPA}{\CNM\shyph\CPA}
% \newcommand{\CNMCCAa}{\CNM\shyph\CCAa}
% \newcommand{\CNMCCAb}{\CNM\shyph\CCAb}


% %%%%%%%%%%%%   reference   %%%%%%%%%%%%%%%%%%
% \newcommand{\namedref}[2]{{#1~\ref{#2}}}
% \newcommand{\chapterref}[1]{\namedref{Chapter}{#1}}
% \newcommand{\sectionref}[1]{\namedref{Section}{#1}}
% \newcommand{\subsectionref}[1]{\namedref{Subsection}{#1}}
% \newcommand{\appendixref}[1]{\namedref{Appendix}{#1}}
% \newcommand{\theoremref}[1]{\namedref{Theorem}{#1}}
% \newcommand{\remarkref}[1]{\namedref{Remark}{#1}}
% \newcommand{\definitionref}[1]{\namedref{Definition}{#1}}
% \newcommand{\lemmaref}[1]{\namedref{Lemma}{#1}}
% \newcommand{\claimref}[1]{\namedref{Claim}{#1}}
% \newcommand{\corollaryref}[1]{\namedref{Corollary}{#1}}
% \newcommand{\constructionref}[1]{\namedref{Construction}{#1}}
% \newcommand{\propertyref}[1]{\namedref{Property}{#1}}
% \newcommand{\protocolref}[1]{\namedref{Protocol}{#1}}
% \newcommand{\algorithmref}[1]{\namedref{Algorithm}{#1}}
% \newcommand{\assumptionref}[1]{\namedref{Assumption}{#1}}
% \newcommand{\figureref}[1]{\namedref{Figure}{#1}}
% \newcommand{\tableref}[1]{\namedref{Table}{#1}}
% \newcommand{\schemeref}[1]{\namedref{Scheme}{#1}}
% \newcommand{\equationref}[1]{{Equation}~(\ref{#1})}
% \newcommand{\propositionref}[1]{\namedref{Proposition}{#1}}
% %
% \newcommand{\jnamedref}[2]{{\ref{#2}~#1}}
% \newcommand{\jsectionref}[1]{\jnamedref{章}{#1}}
% \newcommand{\jsubsectionref}[1]{\jnamedref{節}{#1}}
% \newcommand{\jtheoremref}[1]{\namedref{定理}{#1}}
% \newcommand{\jremarkref}[1]{\namedref{補足}{#1}}
% \newcommand{\jdefinitionref}[1]{\namedref{定義}{#1}}
% \newcommand{\jlemmaref}[1]{\namedref{補題}{#1}}
% \newcommand{\jclaimref}[1]{\namedref{主張}{#1}}
% \newcommand{\jcorollaryref}[1]{\namedref{系}{#1}}
% \newcommand{\jconstructionref}[1]{\namedref{構成}{#1}}
% \newcommand{\jpropertyref}[1]{\namedref{性質}{#1}}
% \newcommand{\jprotocolref}[1]{\namedref{プロトコル}{#1}}
% \newcommand{\jalgorithmref}[1]{\namedref{アルゴリズム}{#1}}
% \newcommand{\jassumptionref}[1]{\namedref{仮定}{#1}}
% \newcommand{\jfigureref}[1]{\namedref{図}{#1}}
% \newcommand{\jtableref}[1]{\namedref{表}{#1}}
% \newcommand{\jschemeref}[1]{\namedref{方式}{#1}}
% \newcommand{\jequationref}[1]{\namedref{式}{#1}}
% \newcommand{\jtabularref}[1]{\namedref{表}{#1}}
% %%%%%%%%     leftright     %%%%%%%%%%%
% \def\（{\left(}
% \def\）{\right)}
% \def\｛{\left\{}
% \def\｝{\right\}}
% \def\［{\left[}
% \def\］{\right]}
% %%%%%%%%   anonymization   %%%%%%%%%
% \newcommand{\Pk}{{\textit{Pk}}}
% \newcommand{\Pert}{\algo{Perturb}}
% %%%%%%%%   distribution   %%%%%%%%%
% \newcommand{\Lap}{\ensuremath{{f_{\text{lap}}}}}
% %%%%%%%%   protocols   %%%%%%%%%
% \newcommand{\Mult}{\protocol{Mult}}
% \newcommand{\Sort}{\protocol{Sort}}
% \newcommand{\Shuffle}{\protocol{Shuffle}}
% \newcommand{\Reveal}{\protocol{Reveal}}
% \newcommand{\Inv}{\protocol{Inv}}



%%%%%%%%   memo   %%%%%%%%

% %---------------------------------------
% % theorem style
% %---------------------------------------
% \newtheorem{jdefinition}{定義}[section]
% \newtheorem{jtheorem}{定理}[section]
% \newtheorem{jlemma}{補題}[section]
% \newtheorem{jcorollary}{系}[section]
% \newcommand{\jproof}{\noindent[{\bf 証明}]~}
% \newcommand{\jsketch}{\noindent[{\bf 証明のスケッチ}]~}
% \newtheorem{definition}{definition}[section]
% \newtheorem{theorem}{theorem}[section]
% \newtheorem{lemma}{lemma}[section]
% \newtheorem{corollary}{corollary}[section]
% \newcommand{\proof}{\noindent[{\bf Proof}]~}
% \newcommand{\sketch}{\noindent[{\bf Sketch of proof}]~}
% %---------------------------------------
% % algorithm, algorithmic
% %---------------------------------------
% \usepackage{algorithm, algorithmic}
% \makeatletter
% \renewcommand{\ALG@name}{Protocol}
% \makeatother
% %---------------------------------------
% \renewcommand{\baselinestretch}{0.86}
% \makeatletter
% \renewenvironment{itemize}%
% {%
% \begin{list}{\parbox{1zw}{$\bullet$}}% 見出し記号／直後の空白を調節
% {%
% \setlength{\topsep}{0.1zh}%itemize始めた時の上との間
% \setlength{\itemindent}{0zw}
% \setlength{\leftmargin}{1.4zw}% 左のインデント
% \setlength{\rightmargin}{0zw}% 右のインデント
% \setlength{\labelsep}{0.2zw}% 黒丸と説明文の間
% \setlength{\labelwidth}{3zw}% ラベルの幅
% \setlength{\itemsep}{0.1em}% 項目ごとの改行幅
% \setlength{\parsep}{0em}% 段落での改行幅
% \setlength{\listparindent}{0zw}% 段落での一字下り
% }
% }{%
% \end{list}%
% }
% \newenvironment{itemize2}%  
% {%
%    \begin{list}{\parbox{1zw}{}}% 見出し記号／直後の空白を調節
%    {%
%       \setlength{\topsep}{2mm}
%       \setlength{\itemindent}{0zw}
%       \setlength{\leftmargin}{1zw}%  左のインデント
%       \setlength{\rightmargin}{0zw}% 右のインデント
%       \setlength{\labelsep}{0.5zw}%    黒丸と説明文の間
%       \setlength{\labelwidth}{4zw}%  ラベルの幅
%       \setlength{\itemsep}{1mm}%     項目ごとの改行幅
%       \setlength{\parsep}{0.2mm}%      段落での改行幅
%       \setlength{\listparindent}{0zw}% 段落での一字下り
%    }
% }{%
%    \end{list}%
% }
% \renewenvironment{enumerate}
% {%
%   \begin{list}{\arabic{enumi}.\ \,}%  見出し記号／直後の空白を調節
%   {%
%      \usecounter{enumi}
%      \setlength{\topsep}{2mm}
%      \setlength{\itemindent}{0zw}%  ここは 0 に固定
%      \setlength{\leftmargin}{1.5zw}%  左のインデント
%      \setlength{\rightmargin}{0zw}% 右のインデント
%      \setlength{\labelsep}{0zw}%    黒丸と説明文の間
%      \setlength{\labelwidth}{3zw}%  ラベルの幅
%      \setlength{\itemsep}{0mm}%     項目ごとの改行幅
%      \setlength{\parsep}{0.2mm}%      段落での改行幅
%      \setlength{\listparindent}{0zw}% 段落での一字下り
%   }
% }{%
%   \end{list}%
% }
% \makeatother
% 

% %%%%%%%%% macro %%%%%%%%%%%%%
% \newcommand{\functionality}[3]{
% \begin{figure}[htbp]
% \centering
% \fbox{
% \begin{minipage}{.9\textwidth}
% \begin{center}
% \textbf{Functionality} {#1F}
% \end{center}
% {#2}
% \end{minipage}
% }
% \caption{#3}
% \end{figure}
% }


